A Practical System for Guaranteed Access in the Presence of DDoS Attacks and Flash Crowds

With the growing incidents of flash crowds and sophisticated DDoS attacks mimicking benign traffic, it becomes challenging to protect Internet-based services solely by differentiating attack traffic from legitimate traffic. While fair-sharing schemes are commonly suggested as a defense when differentiation is difficult, they alone may suffer from highly variable or even unbounded waiting times. We propose RainCheck Filter (RCF), a lightweight primitive that guarantees bounded waiting time for clients despite server flooding without keeping per-client state on the server. RCF achieves strong waiting time guarantees by prioritizing clients based on how long the clients have waited-as if the server maintained a queue in which the clients lined up waiting for service. To avoid keeping state for every incoming client request, the server sends to the client a raincheck, a timestamped cryptographic token that not only informs the client to retry later but also serves as a proof of the client's priority level within the virtual queue. We prove that every client complying with RCF can access the server in bounded time, even under a flash crowd incident or a DDoS attack. Our large-scale simulations confirm that RCF provides a small and predictable maximum waiting time while existing schemes cannot. To demonstrate its deployability, we implement RCF as a Python module such that web developers can protect a critical server resource by adding only three lines of code.

==> extensions.tex <==
%\section{Improvements}\label{sec:extensions}
 %% and independent of the number of bots ($Z$).
\comment{remove some  subsection for now, maybe add in discussion? }
%We demonstrate that \name's MWT guarantees can be further strengthened
%(i.e., a reduced $T$) given auxiliary information about
%clients, and we propose a hybrid solution to improve scalability. % , such as
% (1) distinguishability between bots and legitimate clients and (2)
% non-uniform distribution of bots in the Internet.

%% , and (3) prior association between the client and the server.

%In addition to knowing that the waiting time is bounded, knowing the
%actual waiting time increases users' patience~\cite{Nah2004,
%  Branaghan2009}. To provide users' actual waiting time, we devise a
%server-side algorithm that accurately estimates each client's waiting
%time. Also, we present how \name can be extended so that a client can access the
%server multiple times without having to wait for the waiting time after each
%accepted request.
%This extension is particular useful in Section
%\ref{ssec:http} where \name is applied to http servers.

%\subsection{Strengthening Waiting Time Guarantees}
%% We extend \name to further strengthen the MWT guarantees (i.e.,
%% getting a tighter upper bound on the waiting time) by exploiting
%% auxiliary information about the clients.

%%\paragraph{Distinguishability between bots and legitimate clients.}

%\name treats all clients alike without differentiating bots from
%legitimate clients. By rejecting bot-originated requests, the server
%can shorten the maximum waiting time bound for legitimate clients.

%\newtext{In practice, the server can first filter out bot-originated
%  requests using existing techniques such as CAPTCHAs~\cite{Ahn2003},
%  known blacklists~\cite{composite-blocking-list}, and
%  geo-blocking. Due to the imperfectness of these detection
%  schemes~\cite{Yan2008,Bursztein2011,Bursztein2011SP} and the
%  possiblity of flash crowds, \name can then be applied to bound the
%  waiting time and ensure fair access for the remaining
%  legitimate-looking requests. Note that the filtering process is
%  optional, and \name by itself already provides MWT guarantees. }

%% To identify and block bots, which are automated without human users,
%% the server applies reverse Turing tests, such as
%% CAPTCHAs~\cite{Ahn2003}, to detect human presence. Additionally, the
%% server can identify bots based on known
%% blacklists~\cite{composite-blocking-list}.




%% but such blacklists are likely to be incomplete or out-of-date or
%% inaccurate due to dynamic IPs.


%%\paragraph{The non-uniform distribution of bots in the Internet.}
%%Recent studies on bot population found a skewed distribution of bots:
%%20 ASes host 41\% of bots~\cite{Li2008} and 538 ASes host over 90\% of
%%bots~\cite{Lee2013}. To exploit this fact, the server establishes a baseline of the normal
%%request rate per AS during peacetime (when the server is not flooded),
%%and the baseline is used to allocate resources for each AS, similar to
%%the proportional allocation technique introduced in
%%Section~\ref{ssec:fairness}. By isolating requests originated from
%%different ASes, \name lowers the waiting time bound for clients in a
%%less contaminated AS, as bots in the same AS have to compete among
%%themselves before being able to attack the server. This approach also
%%motivates ISPs to remove bots in their domains, as users have
%%incentives to switch to less-contaminated ISPs.

%% \paragraph{Prior association between the client and the server.}
%% It is common that a client connects to a server more than once over
%% time. For example, a user may access his or her webmail server on an
%% hourly basis, or query an online database regularly.

%% By allowing the server and the client to negotiate the desired MWT
%% guarantee using established connections, \name flexibly supports
%% different levels of service quality for the client's future
%% connections. For example, clients subscribed to be a ``gold'' member
%% will have their requests accepted in one second; ``sliver'' members
%% will have their requests accepted within 5 seconds, etc. The server
%% enforces such guarantees by limiting the number of clients with
%% premium services, and allocating one priority queue for each
%% membership level.

%% After negotiating the MWT guarantee, the server issues to the client a
%% \emph{MWT cookie} that encodes the membership information, such that
%% the server can process the client's future requests according to its
%% membership level without keeping per-client state that needs to be
%% queried before returning a \raincheck.

%% As clients may attempt to manipulate or deliberately re-use old
%% cookies, we need mechanisms to prevent misuse of such cookies (e.g.,
%% using timestamps, keeping probabilistic state).

%% This is, the server may want to prioritize re-establishment requests
%% based on prior history (e.g., give precedence to infrequent
%% connections), i.e., employing certain admission policies to the
%% requests. We may show different guarantees for different admission
%% policies. For example, a certain number of clients can obtain premier
%% services guaranteeing re-connection in the first trial; and some
%% obtain guaranteed re-connection in two trials, etc.

%\subsection{Extension for Better
%  Scalability}\label{ssec:hybrid-solution}
%% \comment{move this to the extension section? HJ: I agree that it may
%%   be a better fit in Section 5.  If we're out of space, we should
%%   maybe move this whole section (except implementation) to appendix. }

%To avoid sudden increase in the bandwidth loads in the rare case when
%all clients retry concurrently, it is desirable to distribute the
%bandwidth loads caused by \raincheck renewals. We propose a hybrid
%scheme that combines \name with a coarse-grained scheduling for
%balancing load distribution.

%% name precisely determines when a client can be served at the cost of
%% possible bandwidth overload if all clients retry concurrently.  Hence
%% it is desirable to distribute the bandwidth loads caused by \raincheck
%% renewals.


% We present a hybrid scheme with improved scalability. This hybrid
% scheme combines \name and a coarse-grained scheduling for retries. The
% main purpose of such coarse-grained scheduling is to distribute the
% bandwidth loads caused by \raincheck renewals across time rather than
% to precisely determine when a client can be served.

%Similar to the original \name, this hybrid scheme requires each client
%to renew its \raincheck periodically. The novel improvement is the
%assignment of the coarse time interval such that all the requests from
%the same client always fall in the same time interval, reducing the
%overhead for duplicate detection and rate limiting.

% this hybrid scheme assigns to each request a coarse time interval
% during which the request should return. More importantly, the
% assignment is designed in a way that requests from the same client
% will fall into the same time interval, reducing the overhead for
% duplicate detection and rate limiting.

%In particular, the server divides the time into non-overlapping time
%intervals
%$\delta_i = [i\cdot w, (i+1)\cdot w)$ for some constant $w$. A \raincheck issued during $\delta_i$ is %valid only
%during $\delta_j$ where $j \in [i+m_{min}, i+m_{max})$ for some
%required cooling period $m_{min}$ and expiration period $m_{max} =
%m_{min} + m_{\Delta}$ ($m_{min}$, $m_{max}$, and $m_{\Delta}$ are
%positive integers). % We explain how to determine $j$ below. We call
% $m_{min}$ the required cooling period and $m_{max} = m_{min} +
% m_{\Delta}$ the expiration period. $m_{min}$, $m_{max}$, and
% $m_{\Delta}$ are positive integers. \comment{any better naming?}
%% We consider such an overlapping division on purpose because
%% non-overlapping intervals may result in non-uniform service
%% utilization---where requests are clustered in the middle of each
%% interval to avoid being falsely declined due to synchronization
%% problems.
% For a request that arrives during $\delta_i$ and is postponed, the
% server provides a \raincheck that is valid during $\delta_{j}$
% only.
%The integer value $j$ is derived such that

%\begin{align}
%& i + m_{min}  \leq j < i + m_{max}, \nonumber\\
%& j \mod m_{\Delta} = PRF_k(cid) \mod m_{\Delta},\nonumber
%\end{align}\\

%where $k$ is a secret key and $PRF$ is a pseudorandom function. These
%equations have a unique solution.

 %% and with at most two solutions. When there
%% are two possible $j$ values, the server consistently picks the smaller
%% (or larger) one.

%This construction ensures that every \raincheck-carrying request from
%the same client always comes back during the same time interval. Also,
%requests are renewed approximately every $m_{\Delta}$ time
%intervals. Therefore, the server only needs to keep track of the
%accepted requests during the current time interval, $\delta_i$, for
%duplicate detection and rate limiting. This hybrid scheme is easier to
%implement as the server does not need to maintain a sliding window of
%$\Delta$ as in the original \name.
%\comment{cut "the server may want to update the secret key" part}
%%The server may want to update the secret key to increase randomness
%%and minimize the risk of
%%key exposure. Suppose the server would like to completely switch to a
%%new key $k'$ from the beginning of $\delta_v$. To ensure a smooth
%%transition, the server chooses to use either the old key or the new
%%key from the beginning of $\delta_{v-m_{max}}$ on a per-request-basis
%%according to the following criterion: if $j < v$ when computing $j$
%%using the old key, use the old key; otherwise use the new key.


%%This hybrid scheme trades flexibility for scalability. At one extreme
%%where the PRF perfectly distributes the clients among $m_{\Delta}$
%%intervals, the overhead (e.g., storage or bandwidth consumed by
%%raincheck renewal) is reduced by an order of $m_{\Delta}$. In
%%particular, we obtain a MWT guarantee $\lceil \frac{N}{L}\rceil w$
%%when $w \geq \frac{L}{R_s}$. We omit this proof since it is similar to
%%that in Section~\ref{sec:analysis}.  At the other extreme where the
%%PRF maps every client to the same time interval, it is degenerated to
%%the original \name with $\Delta = m_{max} \cdot w$, rendering a MWT bound
%%$\lceil \frac{N}{L}\rceil m_{max} w$. Since any practical
%%implementation of PRF should generate reasonably randomized outputs
%%given that the key is kept secret, this hybrid scheme is expected to
%%have much better scalability than the original \name.

%%The server can adjust $m_{max}$ dynamically to distribute the load
%%among $m_{max} - m_{min}$ intervals such that the server is slightly
%%overloaded during each interval. The $m_{min}$ value
%%should be large enough to ensure that requests can return to the
%%server on time.

\section{Waiting Time Estimation}\label{ssec:waiting-time-estimation}
Providing users with feedback of their expected waiting time can
help increase their willingness to wait~\cite{Nah2004, Branaghan2009}. While the
waiting time bound $T$ can serve as a loose estimate of the actual
waiting time, we desire a better estimate that incorporates the
current client status.

We present a \emph{rank estimation} algorithm that allows the server
to estimate any client $c$'s rank (i.e., position in the virtual que)
at time $t$ without keeping per-client state. The algorithm refines
the estimate by taking into account the number of clients that did not
renew their \rainchecks,
% gave up waiting in line (i.e., not renewing
% their \rainchecks).
% This is particularly useful when many requests never reappear (e.g.,
% requests with spoofed addresses).
and the server informs the client the estimated rank by piggybacking
it on the \raincheck.  % Consequently, the client can compute the
% estimated time until its request is accepted % how much
% % more time until the acceptance of its request
% based on its resend strategy.

Efficient and accurate rank estimation is challenging: Counting the
number of issued \rainchecks with a smaller timestamp value than that
of client $c$ is inefficient, as it requires maintaining one counter
for each client. Moreover, since a client can have multiple valid
\rainchecks at hand, the server should prevent counting the same
client twice.

To provide efficient and accurate estimation, our rank estimation
algorithm extends a \emph{probabilistic counting} algorithm proposed
by Flajolet and Martin~\cite{Flajolet1983}, which estimates the number
of distinct items in a set using $O(\log N)$ memory, where $N$ is the
number of distinct items. The probabilistic counting algorithm keeps a
bit vector (referred to as an FM sketch) that is initialized to zeros,
and uses a deterministic function to map an item to the $i$th bit with
probability $1/2^{i}$. A bit is set to 1 if an item is mapped to that
bit. Given an FM sketch $V$ the estimated number of distinct items is
$\tilde{n} = 2^{lsb_0(V)}/0.77351$, where $lsb_0(V)$ is the
lowest-order $0$-bit position of $V$ (zero-based indexing). One can
reduce the estimation error by averaging the results of multiple FM
sketches with different index functions. The FM algorithm guarantees a
bounded error such that $Pr[|\tilde{n}- n| < \epsilon N] > 1 - \delta$
with $O(\frac{\log(2/\delta)}{\epsilon^2})$ number of sketches.

%% Client $c_1$ is in front of client $c_2$ at time $t$ if at time $t$
%% client $c_1$ has a valid raincheck whose timestamp is smaller than any
%% of client $c_2$'s valid raincheck.


%% $c_1$ has a smaller rank than $c_2$ at time $t$, or $c_1 <_t c_2$, if
%% at time $t$ client $c_1$ has a valid raincheck whose timestamp is
%% smaller than any of client $c_2$'s valid raincheck.  Hence, $rank(c, t)
%% \triangleq \lvert \{c' \vert c' <_t c \} \rvert$.

\paragraph{Problem formulation.}
Let $U_{t-\Delta}^t(x)$ contain all clients obtaining at least one
\raincheck with a timestamp $\leq x$ during $[t-\Delta, t)$. Let
$n_{t-\Delta}^t(x)$ be the size of $U_{t-\Delta}^t(x)$. Since a client
in front of $c$ at time $t$ must be in $U_{t-\Delta}^t(TS(\rho_c))$,
$rank(c,t) \leq n_{t-\Delta}^t(TS(\rho_c))$, where $\rho_c$ is client
$c$'s \raincheck that has the smallest timestamp value among all valid
\rainchecks at time $t$ and $TS$ stands for timestamp.
\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{figures/rank-estimation-sketch.eps}
\caption{A rank estimation sketch example.}
\label{fig:rank-estimation-sketch}
\end{figure}

Estimating each client's rank separately using FM sketches requires $O(N \log N)$ memory. In contrast, our rank
estimation algorithm is designed to answer queries such as ``How many
distinct items have a value lower than $x$?'' for any $x$, while
keeping only $O(\log N)$ number of items.

Figure~\ref{fig:rank-estimation-sketch} illustrates how the rank
estimation sketch works and its relationship with FM sketches. The
core idea is as follows: instead of setting a bit to one, we store the
item's value at the mapped position if the value is lower than the
currently stored value at that position. To estimate the number of
items whose value is lower than $x$ for any $x$, we convert this rank
estimation sketch back to an FM sketch where a 1-bit is set if the
corresponding position has a value $< x$. The rank estimation
sketch ensures that the resulting FM sketch is the same as the one we
can get by running the FM algorithm over items with a value lower than
$x$. In our setting, items are \rainchecks, and each \raincheck has a
value which is a timestamp. Two \rainchecks are ``identical'' if they
are from the same client. Hence, using this rank estimation algorithm,
we can estimate $n_{t-\Delta}^t(x)$ for any $x$ given a time interval
$[t- \Delta, t)$.

To estimate a client's rank at time $t_{cur}$ in the virtual queue, the server
maintains a rank estimation sketch and resets it periodically every $\Delta$
time, such that the sketch accounts for intervals $[(i-1)\Delta, i\Delta)$ for
all positive integers $i$. The rank $rank(c, t_{cur})$ can be approximated by
the following:

\[rank(c, t_{cur}) \leq rank(c, i\Delta) \leq n_{(i-1)\Delta}^{i\Delta}(TS(\rho_c)),\]
where $i\Delta \leq t_{cur} < (i+1)\Delta$.

Based on the proof in Section~\ref{ssec:waiting-time-analysis}, $rank(c,
i\Delta) - rank(c, t_{cur})$ $\leq (t_{cur}-i\Delta)R_s$. Also,
$n_{(i-1)\Delta}^{i\Delta}(TS(\rho_c)) - rank(c, i\Delta)$ $\leq \Delta R_s$.
Hence, with $O(\frac{\log(2/\delta)}{\epsilon^2})$ number of sketches, we
ensure that the estimation error is less than $\epsilon N +
(t_{cur}-(i-1)\Delta)R_s \leq \epsilon N + 2 \Delta R_s$ with probability
higher than $1-\delta$.

%\subsection{Accommodating Multiple RainChecks}

%There are applications where multiple \rainchecks may be needed per client. For
%example, if \name is applied to the HTTP protocol and each \raincheck allows
%one HTTP request, multiple \rainchecks would be needed to load a single
%web-page (because a typical web-page requires multiple HTTP requests).

%\name can be extended to accomodate \emph{n}-rainchecks per client to support
%similar cases as above. When a client's raincheck is accepted, at most
%\emph{n-1} additional rainchecks can be renewed or accepted for the same client
%during $\Delta$. That is, at any point in time, the total number of client's
%requests in the server should be less than or equal to \emph{n}. The effects of
%allowing multiple rainchecks on waiting time are evaluated in Section
%\ref{ssec:multi_rc}.

